Attention-based Class-Conditioned Alignment for Multi-Source Domain Adaptation of Object Detectors

Domain adaptation methods for object detection (OD) strive to mitigate the impact of distribution shifts by promoting feature alignment across source and target domains. Multi-source domain adaptation (MSDA) allows leveraging multiple annotated source datasets and unlabeled target data to improve the accuracy and robustness of the detection model. Most state-of-the-art MSDA methods for OD perform feature alignment in a class-agnostic manner. This is challenging since the objects have unique modality information due to variations in object appearance across domains. A recent prototype-based approach proposed a class-wise alignment, yet it suffers from error accumulation caused by noisy pseudo-labels that can negatively affect adaptation with imbalanced data. To overcome these limitations, we propose an attention-based class-conditioned alignment method for MSDA, designed to align instances of each object category across domains. In particular, an attention module combined with an adversarial domain classifier allows learning domain-invariant and class-specific instance representations. Experimental results on multiple benchmarking MSDA datasets indicate that our method outperforms state-of-the-art methods and exhibits robustness to class imbalance, achieved through a conceptually simple class-conditioning strategy. Our code is available at: https://github.com/imatif17/ACIA.

==> junk.tex <==
\begin{comment}
Object Detection(OD) is one of the fundamental problems in Deep Learning and Computer Vision. In recent years several works have been proposed to solve OD\cite{fasterrcnn, detr, yolo}.  The change of distribution can happen due to variations in lightning, weather, or camera angle, etc.  A plethora of methods \cite{adaptive_teacher, Weak-strong, progressive} have been proposed to solve this domain shift problem for object detection with unannotated target data and is normally referred as Unsupervised Domain Adaptation(UDA) for Object Detection(OD). Advarsarial alignment is one of the most common approach to solve this problem. Recently, combining advarsarial alignment with mean-teacher learning have shown to be a promising direction. However, normal UDA assumes that the source data is coming from a single distribution. In real-world the source data might come from multiple different distributions,i.e., and there might be a domain shift among source datasets. This increases the complexity of the detector's  training as we have to tackle the domain shift within the source domain, along with the source and target discrepancy. On the other hand, this setting offers a more comprehensive and adaptable approach to UDA by leveraging the multiple source domains, thereby improving the robustness and generalization capability of models across diverse real-world scenarios. This setting is referred to as Multi-Source Domain Adaptation (MSDA) for OD. 

In the literature, there are three methods for MSDA for OD - DMSN\cite{dmsn}, TRKP\cite{trkp}, and PMT\cite{pmt}. All these methods are using a combination of adversarial training and mean-teacher. DMSN had a common backbone shared across domains while the later part of the network learns domain-specific information and uses adversarial-alignment4 to align the features across domain. TRKP also had the initial part of the network shared across domains, while the detection heads were domain-specific. They relied on domain-disentanglement for the detector's training. PMT uses a Multi-class discriminator to align features across multiple domains %. They also emphasise on the importance of class-conditioned adaptation. For this they relied on by a class and domain specific prototypes and aligning them using contrastive loss. 

The class-conditioned alignment ensures that the learned representations of data from different domains are aligned not just in the feature space, but also in the label space. The visual attributes such as appearance, scale, orientation, and other characteristics of objects can differ between domains. If the distinction is notable the feature alignment becomes challenging \cite{pmt}. The UDA methods for OD deals with this problem by focusing on alignment of prototypical representation of object category across source and target\cite{coursetofine, rpn_alignm, graph_induced}. By doing so they rely directly on the pseudo-labels of the target domains, which are generally extremely noisy. This can cause the performance of the detector to drop. Unlike single source UDA, in MSDA there are multiple source domains available, so for the instance-level alignment we can only focus on aligning source domains, which are labeled. Also, as we align the feature space of all the domains at image-level, we indirectly aligning the instance of target domain also. Among the SOTA MSDA methods for OD only PMT focuses on the class-conditioned adaptation at the instance-level. However, this method has a couple of limitations - 1 - Real-world data are generally not unimodal. In some cases, one-prototypes might be insufficient to store class and domain information. 2 - The prototypes of each class are separated equally but this should be adaptive. For example, cars and trucks are more similar to each other as compared to cars and traffic signs. One way to solve this problem is by having multiple prototypes per object category, calculated using clustering algorithms. But this increases the computational cost as now we have to store all the previous ROI-pooling outputs to calculate the centroid using the clustering algorithm. Also, calculating the number of centroids can be tricky, as the model will be evolving throughout the training.
\end{comment}

\begin{comment}
With the recent advancements, deep ODs have shown impressive results in many object detection benchmarks ranging from closed-world fixed class settings to open-world scenarios \cite{detr, detic-zhou-2022, yolov7-wang-2023, groundingdino-liu-2023}. However, the performance of these detectors degrades if the training (source) and test (target) data are from different distributions (domain shift). Due to that, numerous methods are proposed to improve the detector's performance under domain shifts \cite{adaptive_teacher, strong_weak_alignment, MT_graph, MTunbiased}. These methods are generally referred as Unsupervised Domain Adaptation(UDA) for Object Detection(OD). 

The UDA methods assumes that the source data comes from a single distribution. HoweverBut in a practical scenario, the source dataset can be obtained from multiple sources/sites with considerable domain shifts. For example, factors like weather, geographic location, and illumination can result in source-data discrepancy. This setting is referred to as Multi-Source Domain Adaptation (MSDA) for OD.  Although it is possible to train the model by mixing all the source domain datasets, better results are observed when the source-level discrepancy is modeled explicitly \cite{dmsn, trkp}. This gave rise to the popularity of multi-source domain adaptation techniques \cite{pmt, msda-classif-neurips-2020, adversarial_msda-neurips-2018, coupled-training-msda}. Inspired by the single-source domain adaptation techniques, the typical approach for MSDA involves learning task-specific knowledge from the labeled source dataset, parallelly trying to make the feature space domain-invariant that aids in generalization to the target domain. Different from the classification MSDA, the detection MSDA learns domain-invariant features both at the image level and instance level \cite{pmt, dmsn, trkp}. The training process then strives to achieve the balance between learning feature representations that are invariant to multiple domain shifts while still being discriminative enough to learn to localize individual instances.
\end{comment}






%Different from classification, detection focuses on both classification and localization. This is particularly challenging because objects may appear differently across domains. So unlike classification which primarily focuses on feature alignment, in detection it's also important to align object categories across domains, i.e., class-conditioned adaptation.

%The training process then strives to achieve the balance between learning feature representations that are invariant to multiple domain shifts while still being discriminative enough to learn to localize individual instances.On the other hand, this setting offers a more comprehensive and adaptable approach to UDA by leveraging the multiple source domains, thereby improving the robustness and generalization capability of models across diverse real-world scenarios. This setting is referred to as Multi-Source Domain Adaptation (MSDA) for OD.

%The source dataset itself can be obtained from multiple sources/sites with considerable domain shifts. For example, factors like weather, geographic location, and illumination can result in source-data discrepancy. Although it is possible to train the model by mixing all the source domain datasets, better results are observed when the source-level discrepancy is modeled explicitly \cite{dmsn, trkp}. This gave rise to the popularity of multi-source domain adaptation techniques \cite{pmt, msda-classif-neurips-2020, adversarial_msda-neurips-2018, coupled-training-msda}. Inspired by the single-source domain adaptation techniques, the typical approach for MSDA involves learning task-specific knowledge from the labeled source datasets, parallelly trying to create a domain-invariant feature space that aids the generalization to the target domain. Different from the classification MSDA, the detection MSDA learns domain-invariant features both at the image level (global features) and instance level (local features) \cite{pmt, dmsn, trkp}. The training process then strives to achieve the balance between learning feature representations that are invariant to multiple domain shifts while still being discriminative enough to learn to localize individual instances.


% By using contrastive loss on these prototypes they were able to perform class-conditioned adaptation.
%The common design choice for image-level alignment in MSDA methods is adversarial training by using a class discriminator. For the instance level alignment (domain-invariance at the instance level), existing MSDA methods follow different approaches. DMSN \cite{dmsn} \& TRKP \cite{trkp} (fig. \ref{fig:msda_align_comparison} (a)) utilizes pairwise alignment where each source-target pair of images are aligned with an adversarial loss. They don't use explicit instance-level alignment but instead rely on image-level alignment to get the required domain invariance. PMT (fig. \ref{fig:msda_align_comparison} (b)) observed that doing instance-level alignment in a class-wise fashion improves the performance. They proposed to do instance-level alignment in a two-step fashion, where the first step aligns instances to domain-specific prototypes (in a class-wise fashion using class prototypes for each class in each domain). The second step aligns domain-specific prototypes to domain-invariant prototypes (again in a class-wise fashion). The domain-invariant prototypes for each class are derived from the domain-specific prototypes by simple averaging. 
%However, doing instance-level alignment this way requires a prototype for each class and each source domain, which makes the model sensitive to source domains that are unbalanced or with missing classes. 
%However, this two-step process for instance-level alignment is difficult to realize during training (\textcolor{red}{need better reasoning here}). 



%The superiority of our class-conditioned aligner is illustrated in \cref{fig:tsne_comparison}. The methods without class-wise alignment suffer from severe misalignment (\cref{fig:tsne1}). PMT with prototype-based alignment reduces this misalignment but still suffers for underrepresented classes (the red one in \cref{fig:tsne2}). ACIA with the simplest class-conditioned alignment scheme results in superior alignment across all categories regardless of their abundance (\cref{fig:tsne3}).
%Specifically, we utilize a transformer-based attention module that incorporate class-information into the ROI-Pooled features. The attention scheme uses instance-level features obtained from each domain to compute query and value vectors. The key vectors are obtained from class-label embeddings. The attention output is then used by a domain classifier to do the domain discrimination. The gradients are reversed from the output of the instance-level feature extractor forcing those features to be domain-invariant and class-wise aligned at the same time. This allows a simple but efficient multi-source class-conditional alignment.




\begin{comment}
    
\subsection{Individual class study}

\begin{table*}
    \centering
    \resizebox{.95\textwidth}{!}{% <------ Don't forget this %
      \begin{tabular}{l l l | l l l l l l l l l l | l }
      \hline
    \textbf{Setting} & \textbf{Source} & \textbf{Method}  & \textbf{Bike} & \textbf{Bus} & \textbf{Car} &
    \textbf{Motor} & \textbf{Person} &
    \textbf{Rider} & \textbf{Light} & \textbf{Sign} & \textbf{Train} & \textbf{Truck} & \textbf{mAP}\\ 
    \hline
    \hline
     \multirow{3}{*}{Source Only} & D & \multirow{3}{*}{FRCNN\cite{fasterrcnn}} & 35.1 & 51.7 & 52.6 & 9.9 & 31.9 & 17.8 & 21.6 & 36.3 & - & 47.1 & 30.4
     \\
     & N &  & 27.9 & 32.5 & 49.4 & 15.0 & 28.7 & 21.8 & 14.0 & 30.5 & - & 30.7 & 25.0
     \\
     & D+N &  & 31.5 & 46.9 & 52.9 & 8.4 & 29.5 & 21.6 & 21.7 & 34.3 & - & 42.2 & 28.9
     \\
     \hline

     \multirow{5}{*}{UDA Blending} & \multirow{5}{*}{D+N} & Strong-Weak\cite{strongweak} & 29.7 & 50.0 & 52.9 & 11.0 & 31.4 & 21.1 & 23.3 & 35.1 & - & 44.9 & 29.9
     \\
     &  & Graph Prototype\cite{MT_graph} & 31.7 & 48.8 & 53.9 & 20.8 & 32.0 & 21.6 & 20.5 & 33.7 & - & 43.1 & 30.6
     \\
     &  & Cat. Regularization\cite{categorical} & 25.3 & 51.3 & 52.1 & 17.0 & 33.4 & 18.9 & 20.7 & 34.8 & - & 47.9 & 30.2
     \\
     &  & UMT\cite{MTunbiased} & 42.3 & 48.1 & 56.4 & 13.5 & 35.3 & 26.9 & 31.1 & 41.7 & - & 40.1 & 33.5
     \\
     &  & Adaptive Teacher\cite{adaptive_teacher} & 43.1 & 48.9 & 56.9 & 14.7 & 36.0 & 27.1 & 32.7 & 43.8 & - & 42.7 & 34.6
     \\
     \hline
     
     
     \multirow{6}{*}{MSDA} & \multirow{5}{*}{D+N} & MDAN\cite{MDAN} &  37.1 & 29.9 & 52.8 & 15.8 & 35.1 & 21.6 & 24.7 & 38.8 & - & 20.1 & 27.6
     \\
     & & M$^3$SDA\cite{moment} & 36.9 & 25.9 & 51.9 & 15.1 & 35.7 & 20.5 & 24.7 & 38.1 & - & 15.9 & 26.5
     \\
     & & DMSN\cite{dmsn} & 36.5 & 54.3 & 55.5 & 20.4 & 36.9 & 27.7 & 26.4 & 41.6 & - & 50.8 & 35.0
     \\
     & & TRKP\cite{trkp} & 48.4 & 56.3 & 61.4 & 22.5 & 41.5 & 27.0 & 41.1 & 47.9 & - & 51.9 & 39.8
     \\
     &  & PMT & 55.3  & 59.8  & 67.6  &  29.9  &  47.6 & 32.7  &  46.3   & 56.0  &  -  &  57.7 & 45.3
     \\
     &  & No Class Allign & 56.0  & 57.7  & 66.7  &  33.0  &  47.6 & 31.8  &  46.5   & 54.3  &  -  &  55.1 & 44.9
     \\
     &  & No Class Embed & 51.2  & 57.7  & 67.1  &  31.5  &  48.1 & 37.7  &  45.8   & 55.5  &  -  &  58.4 & 45.3
     \\
     &  & Cross-Entropy & 53.0  & 59.4  & 68.3  &  29.8  &  49.9 & 35.0  &  48.7   & 58.3  &  -  &  58.2 & 46.1
     \\
    &  & \textbf{Ours} & \textbf{56.1}  & \textbf{61.0}  & \textbf{69.2}  &  \textbf{31.9}  &  \textbf{51.8} & \textbf{39.8}  &  \textbf{49.2}   & \textbf{59.0}  &  -  &  \textbf{61.0} & \textbf{47.9}
     \\

    &  & Percentage & .5 & 1 & 57.8 & .2 & 6.5 & .3 & 13.4 & 17.8 & 0 & 2.4 & 100 \\
    \\

    \hline
     \multirow{2}{*}{Oracle} & \multirow{2}{*}{D+N} & Target Only & 27.2  & 39.6  & 51.9   &  12.7  &  29.0 & 15.2  &  20.0   & 33.1  &  -  &  37.5 & 26.6
     \\
      & &  All-Combined & 56.4  & 59.9  & 67.3  &  30.8  &  47.9 & 33.9  &  47.2   & 57.8  &  -  &  54.8 & 45.3
      \\
     \hline
    \end{tabular}% <------ Don't forget this %
    }
    \caption{Class-wise AP of PMT compared against the baseline,
UDA, MSDA, and oracle methods on BDD100K. Source domains
are daytime (D) and night (N) subsets and the target is always
Dusk/Dawn of BDD100K}
    \label{table:Classwise_bdd100k}
\end{table*}
\end{comment}







\begin{comment}
     46.3  & 66.3  & 56.4   &  40.9  & 51.6  & 45.4 &  57.8   &  54.0 & 26.9   &  - & 44.6

     'bbox', {'AP': 23.479323766294268, 'AP50': 45.282507478553626, 'AP75': 21.710942587599675, 'AP50-traffic light': 09911668183574, 'AP50-traffic sign': 56.003151575813604, 'AP50-car': 67.63211348579604, 'AP50-person': 47.680501268005635, 'AP50-bus': , 'AP50-truck': 57.34128209378368, 'AP50-rider': , 'AP50-bike': , 'AP50-motor': , 'AP50-train': 0.0}
\end{comment}

\begin{comment}
    
\begin{table*}
    \centering
    \resizebox{.90\textwidth}{!}{% <------ Don't forget this %
      \begin{tabular}{l l l | l l l l l l l  | l }
      \hline
    \textbf{Setting} & \textbf{Source} & \textbf{Method}  & \textbf{Person} & \textbf{Car}  &
    \textbf{Rider} & \textbf{Truck} &
    \textbf{Motor} & \textbf{Bicycle} & \textbf{Bike} & \textbf{mAP}\\ 
    \hline
    \hline
     \multirow{3}{*}{Source Only} & C & \multirow{3}{*}{FRCNN\cite{fasterrcnn}}  & 26.9 & 44.7 & 22.1 & 17.4 & 17.1 & 18.8 & 16.7 & 23.4
     \\
     & C+M &  & 35.2 & 49.5 & 26.1 & 25.8 & 18.9 & 26.1 & 26.5 & 29.7
     \\
     & C+M+S &  & 36.6 & 49.0 & 22.8 & 24.9 & 26.9 & 28.4 & 27.7 & 30.9
     \\
     \hline

     \multirow{4}{*}{UDA Blending} & \multirow{2}{*}{C+M} & Unbiased Teach.\cite{unbiased_teac} & 30.7 & 28.0 & 3.9 & 11.2 & 19.2 & 17.8 & 18.7 & 18.5
     \\
     &  & Adaptive Teacher\cite{adaptive_teacher} & 31.2 & 31.7 & 15.1 & 16.4 & 17.1 & 20.9 & 27.9 & 22.9
     \\
      & \multirow{2}{*}{C+M+S} & Unbiased Teach.\cite{unbiased_teac} & 32.7 & 39.6 & 6.6 & 21.2 & 21.3 & 25.7 & 28.5 & 25.1
     \\
     &  & Adaptive Teacher\cite{adaptive_teacher} & 36.3 & 42.6 & 19.7 & 23.4 & 24.8 & 27.1 & 33.2 & 29.6
     \\
     \hline
     
     \multirow{4}{*}{MSDA} & \multirow{2}{*}{C+M} &  TRKP\cite{trkp} & 39.2 & 53.2 & 32.4 & 28.7 & 25.5 & 31.1 & 37.4 & 35.3
     \\
     &  & \textbf{PMT(ours)} & 41.1 & 53.5 & 31.2 & 31.9 & 33.7 & 34.9 & 44.6 & 38.7
     \\
      & \multirow{2}{*}{C+M+S} &  TRKP\cite{trkp} & 40.2 & 53.9 & 31.0 & 30.8 & 30.4 & 34.0 & 39.3 & 37.1
     \\
     &  & \textbf{PMT(ours)} & 43.3 & 54.1 & 32.0 & 32.6 & 35.1 & 36.1 & 44.8 & 39.7
     \\
     \hline

     \multirow{3}{*}{Oracle} & \multirow{2}{*}{C+M} &  Target Only & 35.3 & 53.9 & 33.2 & 46.3 & 25.6 & 29.3 & 46.7 & 38.6
     \\
     &  & \multirow{2}{*}{All-Combined} & 40.2 & 60.1 & 47.1 & 60.0 & 29.2 & 36.3 & 56.9 & 47.1
     \\
       & C+M+S &  & 41.7 & 63.9 & 49.5 & 58.1 & 31.6 & 39.1 & 53.5 & 48.2
     \\
     \hline
    \end{tabular}% <------ Don't forget this %
    }
    \caption{Class-wise AP of PMT compared against the baselines on Daytime domain of BDD100K. C, M, and S refer to Cityscapes, MS COCO, and Synscapes datasets.}
    \label{table:Classwise_mixed}
\end{table*}

\end{comment}




\begin{comment}

\begin{table*}
    \centering
    \resizebox{.95\textwidth}{!}{% <------ Don't forget this %
      \begin{tabular}{ l | l l l l l l l l l l | l }
      \hline
    \textbf{Method}  & \textbf{Bike} & \textbf{Bus} & \textbf{Car} & \textbf{Motor} & \textbf{Person} & \textbf{Rider} & \textbf{Light} & \textbf{Sign} & \textbf{Train} & \textbf{Truck} & \textbf{mAP}\\ 
    \hline
    \hline
    Percentage & .5 & 1 & 57.8 & .2 & 6.5 & .3 & 13.4 & 17.8 & 0 & 2.4 & 100 \\
    \hline
    \hline
    PMT &  43.8  & 52.3  & -  &  28.0  &  - & 34.4  &  -   &  -  &  -  &  - & 39.6
    Ours & 45.8  & 48.9  & -  &  30.7  &  - & 31.0  &  -   &  -  &  -  &  - & 39.1
    \hline
    PMT & 42.1  & 52.7  & -  &  25.1  &  43.1 & 34.0  &  -   & -  &  -  &  50.5 & 41.2
    Ours & 44.3  & 54.2  & -  &  25.3  &  45.3 & 40.6  &  -   & -  &  -  &  50.4 & 43.4
    \hline
    PMT & 42.1  & 52.7  & -  &  25.3  &  - & 40.6  &  -   & -  &  -  &  50.4 & 43.4
    Ours & 44.3  & 54.2  & -  &  25.1  &  - & 34.0  &  -   & -  &  -  &  50.5 & 41.2
    \hline
    PMT & 55.3  & 59.8  & 67.6  &  29.9  &  47.6 & 32.7  &  46.3   & 56.0  &  -  &  57.7 & 45.3
    \textbf{Ours} & \textbf{56.1}  & \textbf{61.0}  & \textbf{69.2}  &  \textbf{31.9}  &  \textbf{51.8} & \textbf{39.8}  &  \textbf{49.2}   & \textbf{59.0}  &  -  &  \textbf{61.0} & \textbf{47.9}
    


    \end{tabular}% <------ Don't forget this %
    }
    \caption{...}
    \label{table:Classwise_bdd100k}
\end{table*}



\begin{table*}
    \centering
    \resizebox{.95\textwidth}{!}{% <------ Don't forget this %
      \begin{tabular}{ l | l l l l l l l l l l | l }
      \hline
    \textbf{Method}  & \textbf{Bike - .5} & \textbf{Bus - 1} & \textbf{Car - 57.8} & \textbf{Motor - .2} & \textbf{Person - 6.5} & \textbf{Rider - .3} & \textbf{Light - 13.4} & \textbf{Sign - 17.8} & \textbf{Train - 0} & \textbf{Truck - 2.4} & \textbf{mAP}\\ 
    \hline
    \hline
    PMT &  43.8  & 52.3  & -  &  28.0  &  - & 34.4  &  -   &  -  &  -  &  - & 39.6
    Ours & 45.8  & 48.9  & -  &  30.7  &  - & 31.0  &  -   &  -  &  -  &  - & 39.1
    \hline
    PMT & 42.1  & 52.7  & -  &  25.1  &  43.1 & 34.0  &  -   & -  &  -  &  50.5 & 41.2
    Ours & 44.3  & 54.2  & -  &  25.3  &  45.3 & 40.6  &  -   & -  &  -  &  50.4 & 43.4
    \hline
    PMT & 42.1  & 52.7  & -  &  25.3  &  - & 40.6  &  -   & -  &  -  &  50.4 & 43.4
    Ours & 44.3  & 54.2  & -  &  25.1  &  - & 34.0  &  -   & -  &  -  &  50.5 & 41.2
    \hline
    PMT & 55.3  & 59.8  & 67.6  &  29.9  &  47.6 & 32.7  &  46.3   & 56.0  &  -  &  57.7 & 45.3
    \textbf{Ours} & \textbf{56.1}  & \textbf{61.0}  & \textbf{69.2}  &  \textbf{31.9}  &  \textbf{51.8} & \textbf{39.8}  &  \textbf{49.2}   & \textbf{59.0}  &  -  &  \textbf{61.0} & \textbf{47.9}
    


    \end{tabular}% <------ Don't forget this %
    }
    \caption{...}
    \label{table:Classwise_bdd100k}
\end{table*}



\begin{table*}
    \centering
    \resizebox{.95\textwidth}{!}{% <------ Don't forget this %
      \begin{tabular}{ l | l l l l l l l l l l | l }
      \hline
    \textbf{Method}  & \textbf{Bike - .5} & \textbf{Bus - 1}  & \textbf{Motor - .2} & \textbf{Person - 6.5} & \textbf{Rider - .3} &  \textbf{Train - 0} & \textbf{Truck - 2.4} &\textbf{Light - 13.4} & \textbf{Sign - 17.8} & \textbf{Car - 57.8} & \textbf{mAP}\\ 
    \hline
    \hline
    PMT &  43.8  & 52.3   &  28.0  &  - & 34.4  &    -  &  - &  - &  -   &  -  & 39.6
    Ours & 45.8  & 48.9   &  30.7  &  - & 31.0  &    -  &  - &  - &  -   &  -    &  39.1
    \hline
    PMT & 42.1  & 52.7    &  25.1  &  43.1 & 34.0   &  -  &  50.5 & - & -   &  -  &  41.2
    Ours & 44.3  & 54.2    &  25.3  &  45.3 & 40.6   &  -  &  50.4 & - & -   &  -  &  43.4
    \hline
    PMT & 42.1  & 52.7   &  25.3  &  -  &  40.6   &  -  &  50.4 & - &  -   & - &  43.4
    Ours & 44.3  & 54.2   &  25.1  &  - &  34.0   &  -  &  50.5 & - &  -   & - & 41.2
    \hline
    PMT & 55.3  & 59.8   &  29.9  &  47.6 & 32.7  &   -  &  57.7 & 46.3   & 56.0  & 67.6 & 45.3
    \textbf{Ours} & \textbf{56.1}  & \textbf{61.0}  & \textbf{69.2}  &  \textbf{31.9}  &  \textbf{51.8} & \textbf{39.8}  &  -  &  \textbf{61.0} & \textbf{69.2} & \textbf{49.2}   & \textbf{59.0}  & & \textbf{47.9}
    


    \end{tabular}% <------ Don't forget this %
    }
    \caption{...}
    \label{table:Classwise_bdd100k}
\end{table*}




PMT - 6
"bbox/AP50": 41.280754535370896, "bbox/AP50-bike": 42.13759163511869, "bbox/AP50-bus": 52.74603362060405, "bbox/AP50-motor": 25.1202291616235, "bbox/AP50-person": 43.12197761759064, "bbox/AP50-rider": 34.07921156253172, "bbox/AP50-truck": 50.47948361475678

Our - 6 
"bbox/AP50": 43.38623729728647, "bbox/AP50-bike": 44.33602595846606, "bbox/AP50-bus": 54.19482174294416, "bbox/AP50-motor": 25.32067611319536, "bbox/AP50-person": 45.38700942664266, "bbox/AP50-rider": 40.65731546781471, "bbox/AP50-truck": 50.421575074655834


rider', 'bus', 'motor', 'bike'


    
\end{comment}

\begin{comment}
In our proposed method, ACCD is used to perform class-conditioned feature alignment at the instance level. The class-conditioned alignment is important because - 1 - The visual attributes such as appearance, scale, orientation, and other characteristics of objects can differ between domains. If the distinction is notable the feature alignment becomes challenging \cite{pmt}. 2 - It addresses the issue of class imbalance between the domains. It allows the model to focus on adapting specific classes that might be underrepresented in one of the domains. In OD the instance-level alignment is performed after the ROI-Pooling layer. This is different from the image-level alignment as at the instance level we have features of a single object category. From the previous works in DA, we are aware that an adversarial discriminator can perform feature alignment. If we can integrate class information into the features, this feature alignment will be class-conditioned. The class information is available for the source domain because of the annotations. For the target domain, we can use the filtered pseudo-labels generated by the teacher model. However, we found that using the pseudo-labels harms the model's performance. This is because the pseudo-labels are noisy, even after filtering. So, aligning the incorrect bounding box affects the model negatively. That's why we only use the source domains for class alignment. 
\begin{figure}
	\centering 
	%\fbox
        {
		\includegraphics[width=.90\textwidth]{images/class-wise-crop.pdf}
	}
     \\ \parbox{.98\textwidth}{\caption{Class-conditioned alignment for MSDA of OD. For every ROI-pool object feature two projections are created, used as Query (Q) and Value (V) for the attention block. The Key (K) vector is obtained from the embedding layer.} \label{fig:class_disc}}
\end{figure}
\end{comment}
